Implicit Channel Charting with Application to UAV-aided Localization

Traditional localization algorithms based on features such as time difference of arrival are impaired by non-line of sight propagation, which negatively affects the consistency that they expect among distance estimates. Instead, fingerprinting localization is robust to these propagation conditions but requires the costly collection of large data sets. To alleviate these limitations, the present paper capitalizes on the recently-proposed notion of channel charting to learn the geometry of the space that contains the channel state information (CSI) measurements collected by the nodes to be localized. The proposed algorithm utilizes a deep neural network that learns distances between pairs of nodes using their measured CSI. Unlike standard channel charting approaches, this algorithm directly works with the physical geometry and therefore only implicitly learns the geometry of the radio domain. Simulation results demonstrate that the proposed algorithm outperforms its competitors and allows accurate localization in emergency scenarios using an unmanned aerial vehicle.

==> pdflatex <==
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
** ATTENTION: Single column mode is not typically used with IEEE publications.
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-bibtex.def

Package biblatex Warning: Using fall-back BibTeX(8) backend:
(biblatex)                functionality may be reduced/unavailable.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/alphabetic.bbx
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/standard.bbx))
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/cbx/alphabetic.cbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/lbx/english.lbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3kernel/expl3.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-2020-10-
01.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-generic.
tex)))) (./draft.bbl

Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'agostini2020channel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2018deep':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2019novel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020feature':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020triplet':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'huang2019improving':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'kaski2003trustworthiness':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'li2019massive':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'niitsoo2018convolutional':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'patwari2008nesh':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'romero2022aerial':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sammon1969mapping':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'savvides2001dynamic':
(biblatex)                - Can't use 'location' + 'address' 
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'studer2018charting':
(biblatex)                - Invalid format of field 'month'.

) (/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.

Overfull \hbox (37.33464pt too wide) in paragraph at lines 207--230
[][]$[]$[]\OT1/ptm/m/n/10 More so-phis-ti-cated al-ter-na-tives rely on deep ne
u-ral net-works (DNNs) to learn a map-ping from CSI [[]arnold2018deep[];
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2]
Overfull \hbox (4.45522pt too wide) in paragraph at lines 443--448
[][]$[]$[]\OT1/ptm/m/n/10 (i) ex-ist-ing schemes for lo-cal-iza-tion with UAVs 
rely on model-

LaTeX Warning: Reference `sec:simulation' on page 3 undefined on input line 477
.


LaTeX Warning: Reference `sec:conclusion' on page 3 undefined on input line 479
.

[3] [4 <./figs/Fig.ecc_icc.pdf> <./figs/Fig.city_map.pdf>] [5]

LaTeX Warning: Reference `sec:simulation' on page 6 undefined on input line 866
.

[6 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>]

LaTeX Warning: Reference `eq:ls_problem' on page 7 undefined on input line 963.


[7]

LaTeX Warning: Reference `fig:rmse_anchors' on page 8 undefined on input line 1
064.


LaTeX Warning: Citation 'sobehy2020nearest' on page 8 undefined on input line 1
085.

[8 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>]
Overfull \hbox (4.61969pt too wide) in paragraph at lines 1143--1143
\OT1/ptm/m/n/10 graphic Maps''. In: \OT1/ptm/m/it/10 IEEE Int. Conf. Acous-tics
 Speech Sig-nal Pro-cess. Avail-able at arXiv:2109.07372\OT1/ptm/m/n/10 .
[9] [10] (./draft.aux)

LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `draft.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.


Package biblatex Warning: Please (re)run BibTeX on the file(s):
(biblatex)                draft
(biblatex)                and rerun LaTeX afterwards.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfont
s/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/
utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb
></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (10 pages, 781441 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
** ATTENTION: Single column mode is not typically used with IEEE publications.
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-bibtex.def

Package biblatex Warning: Using fall-back BibTeX(8) backend:
(biblatex)                functionality may be reduced/unavailable.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/alphabetic.bbx
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/standard.bbx))
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/cbx/alphabetic.cbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/lbx/english.lbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3kernel/expl3.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-2020-10-
01.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-generic.
tex)))) (./draft.bbl

Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'agostini2020channel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2018deep':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2019novel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020feature':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020triplet':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'huang2019improving':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'kaski2003trustworthiness':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'li2019massive':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'niitsoo2018convolutional':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'patwari2008nesh':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'romero2022aerial':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sammon1969mapping':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'savvides2001dynamic':
(biblatex)                - Can't use 'location' + 'address' 
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sobehy2020nearest':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'studer2018charting':
(biblatex)                - Invalid format of field 'month'.

) (/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.

Overfull \hbox (37.33464pt too wide) in paragraph at lines 207--230
[][]$[]$[]\OT1/ptm/m/n/10 More so-phis-ti-cated al-ter-na-tives rely on deep ne
u-ral net-works (DNNs) to learn a map-ping from CSI [[]arnold2018deep[];
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2]
Overfull \hbox (4.45522pt too wide) in paragraph at lines 443--448
[][]$[]$[]\OT1/ptm/m/n/10 (i) ex-ist-ing schemes for lo-cal-iza-tion with UAVs 
rely on model-
[3] [4 <./figs/Fig.ecc_icc.pdf> <./figs/Fig.city_map.pdf>] [5] [6 <./figs/Fig.h
igh_level.pdf> <./figs/Fig.detailed_level.pdf>] [7] [8 <./figs/Fig.rmse_vs_anch
ors.pdf> <./figs/Fig.rmse_vs_noise.pdf>]
Overfull \hbox (4.61969pt too wide) in paragraph at lines 1143--1143
\OT1/ptm/m/n/10 graphic Maps''. In: \OT1/ptm/m/it/10 IEEE Int. Conf. Acous-tics
 Speech Sig-nal Pro-cess. Avail-able at arXiv:2109.07372\OT1/ptm/m/n/10 .
[9] [10] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfont
s/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/
utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb
></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (10 pages, 780135 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
** ATTENTION: Single column mode is not typically used with IEEE publications.
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-bibtex.def

Package biblatex Warning: Using fall-back BibTeX(8) backend:
(biblatex)                functionality may be reduced/unavailable.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/alphabetic.bbx
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/standard.bbx))
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/cbx/alphabetic.cbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/lbx/english.lbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3kernel/expl3.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-2020-10-
01.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-generic.
tex)))) (./draft.bbl

Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'agostini2020channel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2018deep':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2019novel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020feature':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020triplet':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'huang2019improving':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'kaski2003trustworthiness':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'li2019massive':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'niitsoo2018convolutional':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'patwari2008nesh':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'romero2022aerial':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sammon1969mapping':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'savvides2001dynamic':
(biblatex)                - Can't use 'location' + 'address' 
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sobehy2020nearest':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'studer2018charting':
(biblatex)                - Invalid format of field 'month'.

) (/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.

Overfull \hbox (37.33464pt too wide) in paragraph at lines 207--230
[][]$[]$[]\OT1/ptm/m/n/10 More so-phis-ti-cated al-ter-na-tives rely on deep ne
u-ral net-works (DNNs) to learn a map-ping from CSI [[]arnold2018deep[];
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2]
Overfull \hbox (4.45522pt too wide) in paragraph at lines 443--448
[][]$[]$[]\OT1/ptm/m/n/10 (i) ex-ist-ing schemes for lo-cal-iza-tion with UAVs 
rely on model-
[3] [4 <./figs/Fig.ecc_icc.pdf> <./figs/Fig.city_map.pdf>] [5] [6 <./figs/Fig.h
igh_level.pdf> <./figs/Fig.detailed_level.pdf>] [7] [8 <./figs/Fig.rmse_vs_anch
ors.pdf> <./figs/Fig.rmse_vs_noise.pdf>]
Overfull \hbox (4.61969pt too wide) in paragraph at lines 1144--1144
\OT1/ptm/m/n/10 graphic Maps''. In: \OT1/ptm/m/it/10 IEEE Int. Conf. Acous-tics
 Speech Sig-nal Pro-cess. Avail-able at arXiv:2109.07372\OT1/ptm/m/n/10 .
[9] [10] (./draft.aux)

LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfont
s/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/
utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb
></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (10 pages, 780100 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
** ATTENTION: Single column mode is not typically used with IEEE publications.
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-bibtex.def

Package biblatex Warning: Using fall-back BibTeX(8) backend:
(biblatex)                functionality may be reduced/unavailable.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/alphabetic.bbx
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/standard.bbx))
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/cbx/alphabetic.cbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/lbx/english.lbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3kernel/expl3.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-2020-10-
01.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-generic.
tex)))) (./draft.bbl

Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'agostini2020channel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2018deep':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2019novel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020feature':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020triplet':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'huang2019improving':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'kaski2003trustworthiness':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'li2019massive':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'niitsoo2018convolutional':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'patwari2008nesh':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'romero2022aerial':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sammon1969mapping':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'savvides2001dynamic':
(biblatex)                - Can't use 'location' + 'address' 
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sobehy2020nearest':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'studer2018charting':
(biblatex)                - Invalid format of field 'month'.

) (/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.

Overfull \hbox (37.33464pt too wide) in paragraph at lines 207--230
[][]$[]$[]\OT1/ptm/m/n/10 More so-phis-ti-cated al-ter-na-tives rely on deep ne
u-ral net-works (DNNs) to learn a map-ping from CSI [[]arnold2018deep[];
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2]
Overfull \hbox (4.45522pt too wide) in paragraph at lines 443--448
[][]$[]$[]\OT1/ptm/m/n/10 (i) ex-ist-ing schemes for lo-cal-iza-tion with UAVs 
rely on model-
[3] [4 <./figs/Fig.ecc_icc.pdf> <./figs/Fig.city_map.pdf>] [5] [6 <./figs/Fig.h
igh_level.pdf> <./figs/Fig.detailed_level.pdf>] [7]

LaTeX Warning: Reference `sec:training' on page 8 undefined on input line 1118.



Overfull \hbox (15.27417pt too wide) in paragraph at lines 1113--1126
[][]$[]$[]\OT1/ptm/m/n/10 Incidentally, DFPL is seen to out-per-form NFPL. This
 phe-nomenon has al-ready been ob-served in [[]sobehy2020nearest[]]
[8 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>]
Overfull \hbox (4.61969pt too wide) in paragraph at lines 1162--1162
\OT1/ptm/m/n/10 graphic Maps''. In: \OT1/ptm/m/it/10 IEEE Int. Conf. Acous-tics
 Speech Sig-nal Pro-cess. Avail-able at arXiv:2109.07372\OT1/ptm/m/n/10 .
[9] [10] (./draft.aux)

LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfont
s/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/
utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb
></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (10 pages, 781258 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
** ATTENTION: Single column mode is not typically used with IEEE publications.
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-bibtex.def

Package biblatex Warning: Using fall-back BibTeX(8) backend:
(biblatex)                functionality may be reduced/unavailable.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/alphabetic.bbx
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/bbx/standard.bbx))
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/cbx/alphabetic.cbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/biblatex.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/lbx/english.lbx)
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3kernel/expl3.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-2020-10-
01.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3packages/xparse/xparse-generic.
tex)))) (./draft.bbl

Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'agostini2020channel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2018deep':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'arnold2019novel':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020feature':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'ferrand2020triplet':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'huang2019improving':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'kaski2003trustworthiness':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'li2019massive':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'niitsoo2018convolutional':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'patwari2008nesh':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'romero2022aerial':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sammon1969mapping':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'savvides2001dynamic':
(biblatex)                - Can't use 'location' + 'address' 
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'sobehy2020nearest':
(biblatex)                - Invalid format of field 'month'.


Package biblatex Warning: BibTeX reported the following issues
(biblatex)                with 'studer2018charting':
(biblatex)                - Invalid format of field 'month'.

) (/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.

Overfull \hbox (37.33464pt too wide) in paragraph at lines 207--230
[][]$[]$[]\OT1/ptm/m/n/10 More so-phis-ti-cated al-ter-na-tives rely on deep ne
u-ral net-works (DNNs) to learn a map-ping from CSI [[]arnold2018deep[];
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2]
Overfull \hbox (4.45522pt too wide) in paragraph at lines 443--448
[][]$[]$[]\OT1/ptm/m/n/10 (i) ex-ist-ing schemes for lo-cal-iza-tion with UAVs 
rely on model-
[3] [4 <./figs/Fig.ecc_icc.pdf> <./figs/Fig.city_map.pdf>] [5] [6 <./figs/Fig.h
igh_level.pdf> <./figs/Fig.detailed_level.pdf>] [7]
Overfull \hbox (15.27417pt too wide) in paragraph at lines 1113--1126
[][]$[]$[]\OT1/ptm/m/n/10 Incidentally, DFPL is seen to out-per-form NFPL. This
 phe-nomenon has al-ready been ob-served in [[]sobehy2020nearest[]]
[8 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>]
Overfull \hbox (4.61969pt too wide) in paragraph at lines 1162--1162
\OT1/ptm/m/n/10 graphic Maps''. In: \OT1/ptm/m/it/10 IEEE Int. Conf. Acous-tics
 Speech Sig-nal Pro-cess. Avail-able at arXiv:2109.07372\OT1/ptm/m/n/10 .
[9] [10] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/cm/cmsy9.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfont
s/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/
utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb
></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (10 pages, 780238 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
No file draft.aux.
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty))
** WARNING: \thanks is locked out when in conference mode (line 97).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.

LaTeX Warning: Citation `xiao2022integrated' on page 1 undefined on input line 
159.


LaTeX Warning: Citation `savvides2001dynamic' on page 1 undefined on input line
 163.


LaTeX Warning: Citation `arnold2018deep' on page 1 undefined on input line 209.



LaTeX Warning: Citation `arnold2019novel' on page 1 undefined on input line 209
.


LaTeX Warning: Citation `niitsoo2018convolutional' on page 1 undefined on input
 line 211.


LaTeX Warning: Citation `li2019massive' on page 1 undefined on input line 211.


LaTeX Warning: Citation `ferrand2020feature' on page 1 undefined on input line 
211.


LaTeX Warning: Citation `studer2018charting' on page 1 undefined on input line 
243.


LaTeX Warning: Reference `fig:ecc_workflow' on page 1 undefined on input line 2
62.


LaTeX Warning: Reference `sec:preliminary' on page 1 undefined on input line 27
2.


LaTeX Warning: Citation `huang2019improving' on page 1 undefined on input line 
280.


LaTeX Warning: Citation `studer2018charting' on page 1 undefined on input line 
304.


LaTeX Warning: Citation `ferrand2020triplet' on page 1 undefined on input line 
304.


LaTeX Warning: Citation `bromley1993signature' on page 1 undefined on input lin
e 323.

[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]

LaTeX Warning: Reference `sec:preliminary' on page 2 undefined on input line 46
9.


LaTeX Warning: Reference `sec:problem_formualation' on page 2 undefined on inpu
t line 471.


LaTeX Warning: Reference `sec:ICCL' on page 2 undefined on input line 474.


LaTeX Warning: Reference `sec:simulation' on page 2 undefined on input line 477
.


LaTeX Warning: Reference `sec:conclusion' on page 2 undefined on input line 479
.


LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
511.


LaTeX Warning: Citation `ferrand2020triplet' on page 2 undefined on input line 
522.


LaTeX Warning: Reference `fig:ecc_workflow' on page 2 undefined on input line 5
32.


LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
547.


LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
557.


LaTeX Warning: Citation `agostini2020channel' on page 2 undefined on input line
 558.


LaTeX Warning: Citation `sammon1969mapping' on page 2 undefined on input line 5
65.


LaTeX Warning: Citation `pearson1901liii' on page 2 undefined on input line 568
.


LaTeX Warning: Citation `hotelling1933analysis' on page 2 undefined on input li
ne 568.


LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
569.


LaTeX Warning: Citation `venna2001neighborhood' on page 2 undefined on input li
ne 578.


LaTeX Warning: Citation `kaski2003trustworthiness' on page 2 undefined on input
 line 578.


LaTeX Warning: Citation `vathy2013graph' on page 2 undefined on input line 578.



LaTeX Warning: Citation `huang2019improving' on page 2 undefined on input line 
587.

[2 <./figs/Fig.ecc_icc.pdf>]

LaTeX Warning: Reference `fig:city_map' on page 3 undefined on input line 648.


LaTeX Warning: Citation `savvides2001dynamic' on page 3 undefined on input line
 721.


LaTeX Warning: Reference `fig:ecc_workflow' on page 3 undefined on input line 7
26.


LaTeX Warning: Reference `eq:rxsignal' on page 3 undefined on input line 746.


LaTeX Warning: Citation `kay1' on page 3 undefined on input line 757.


LaTeX Warning: Reference `eq:rxsignal' on page 3 undefined on input line 775.


LaTeX Warning: Reference `eq:estdist' on page 3 undefined on input line 782.


LaTeX Warning: Reference `eq:ggen' on page 3 undefined on input line 791.


LaTeX Warning: Reference `eq:rxsignal' on page 3 undefined on input line 793.


LaTeX Warning: Reference `eq:hestimator' on page 3 undefined on input line 794.


[3 <./figs/Fig.city_map.pdf>]

LaTeX Warning: Reference `fig:high_level' on page 4 undefined on input line 859
.


LaTeX Warning: Reference `fig:low_level' on page 4 undefined on input line 864.



LaTeX Warning: Reference `sec:simulation' on page 4 undefined on input line 866
.


Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;

LaTeX Warning: Reference `sec:intro' on page 4 undefined on input line 901.


LaTeX Warning: Citation `savvides2001dynamic' on page 4 undefined on input line
 929.


Overfull \hbox (65.78949pt too wide) detected at line 963
[]
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>]

LaTeX Warning: Reference `eq:ls_problem' on page 5 undefined on input line 965.



LaTeX Warning: Reference `sec:csiextraction' on page 5 undefined on input line 
983.


LaTeX Warning: Reference `fig:city_map' on page 5 undefined on input line 993.


LaTeX Warning: Citation `patwari2008nesh' on page 5 undefined on input line 994
.


LaTeX Warning: Citation `romero2022aerial' on page 5 undefined on input line 99
5.


LaTeX Warning: Reference `sec:intro' on page 5 undefined on input line 1010.


LaTeX Warning: Citation `arnold2018deep' on page 5 undefined on input line 1025
.


LaTeX Warning: Citation `arnold2019novel' on page 5 undefined on input line 102
5.


LaTeX Warning: Citation `niitsoo2018convolutional' on page 5 undefined on input
 line 1025.


LaTeX Warning: Citation `li2019massive' on page 5 undefined on input line 1025.



LaTeX Warning: Citation `ferrand2020feature' on page 5 undefined on input line 
1025.


LaTeX Warning: Reference `sec:csiextraction' on page 5 undefined on input line 
1027.


LaTeX Warning: Reference `sec:architecture' on page 5 undefined on input line 1
030.


LaTeX Warning: Reference `fig:rmse_anchors' on page 5 undefined on input line 1
067.


LaTeX Warning: Reference `fig:noise' on page 5 undefined on input line 1093.


LaTeX Warning: Citation `sobehy2020nearest' on page 5 undefined on input line 1
115.


LaTeX Warning: Reference `sec:training' on page 5 undefined on input line 1118.



LaTeX Warning: Citation `ferrand2020feature' on page 5 undefined on input line 
1119.


LaTeX Warning: Citation `arnold2018deep' on page 5 undefined on input line 1124
.


LaTeX Warning: Citation `arnold2019novel' on page 5 undefined on input line 112
4.


LaTeX Warning: Citation `niitsoo2018convolutional' on page 5 undefined on input
 line 1124.


LaTeX Warning: Citation `li2019massive' on page 5 undefined on input line 1124.


[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>]
No file draft.bbl.

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (2.16492pt too high) has occurred while \output is active
[6] (./draft.aux)

LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `draft.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 758228 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 97).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.

LaTeX Warning: Citation `xiao2022integrated' on page 1 undefined on input line 
159.


LaTeX Warning: Citation `savvides2001dynamic' on page 1 undefined on input line
 163.


LaTeX Warning: Citation `arnold2018deep' on page 1 undefined on input line 209.



LaTeX Warning: Citation `arnold2019novel' on page 1 undefined on input line 209
.


LaTeX Warning: Citation `niitsoo2018convolutional' on page 1 undefined on input
 line 211.


LaTeX Warning: Citation `li2019massive' on page 1 undefined on input line 211.


LaTeX Warning: Citation `ferrand2020feature' on page 1 undefined on input line 
211.


LaTeX Warning: Citation `studer2018charting' on page 1 undefined on input line 
243.


LaTeX Warning: Citation `huang2019improving' on page 1 undefined on input line 
280.


LaTeX Warning: Citation `studer2018charting' on page 1 undefined on input line 
304.


LaTeX Warning: Citation `ferrand2020triplet' on page 1 undefined on input line 
304.


LaTeX Warning: Citation `bromley1993signature' on page 1 undefined on input lin
e 323.

[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]

LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
511.


LaTeX Warning: Citation `ferrand2020triplet' on page 2 undefined on input line 
522.


LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
547.


LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
557.


LaTeX Warning: Citation `agostini2020channel' on page 2 undefined on input line
 558.


LaTeX Warning: Citation `sammon1969mapping' on page 2 undefined on input line 5
65.


LaTeX Warning: Citation `pearson1901liii' on page 2 undefined on input line 568
.


LaTeX Warning: Citation `hotelling1933analysis' on page 2 undefined on input li
ne 568.


LaTeX Warning: Citation `studer2018charting' on page 2 undefined on input line 
569.


LaTeX Warning: Citation `venna2001neighborhood' on page 2 undefined on input li
ne 578.


LaTeX Warning: Citation `kaski2003trustworthiness' on page 2 undefined on input
 line 578.


LaTeX Warning: Citation `vathy2013graph' on page 2 undefined on input line 578.



LaTeX Warning: Citation `huang2019improving' on page 2 undefined on input line 
587.

[2 <./figs/Fig.ecc_icc.pdf>]

LaTeX Warning: Citation `savvides2001dynamic' on page 3 undefined on input line
 721.


LaTeX Warning: Citation `kay1' on page 3 undefined on input line 757.

[3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;

LaTeX Warning: Citation `savvides2001dynamic' on page 4 undefined on input line
 929.


Overfull \hbox (65.78949pt too wide) detected at line 963
[]
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>]

LaTeX Warning: Citation `patwari2008nesh' on page 5 undefined on input line 994
.


LaTeX Warning: Citation `romero2022aerial' on page 5 undefined on input line 99
5.


LaTeX Warning: Citation `arnold2018deep' on page 5 undefined on input line 1025
.


LaTeX Warning: Citation `arnold2019novel' on page 5 undefined on input line 102
5.


LaTeX Warning: Citation `niitsoo2018convolutional' on page 5 undefined on input
 line 1025.


LaTeX Warning: Citation `li2019massive' on page 5 undefined on input line 1025.



LaTeX Warning: Citation `ferrand2020feature' on page 5 undefined on input line 
1025.


LaTeX Warning: Citation `sobehy2020nearest' on page 5 undefined on input line 1
115.


LaTeX Warning: Citation `ferrand2020feature' on page 5 undefined on input line 
1119.


LaTeX Warning: Citation `arnold2018deep' on page 5 undefined on input line 1124
.


LaTeX Warning: Citation `arnold2019novel' on page 5 undefined on input line 112
4.


LaTeX Warning: Citation `niitsoo2018convolutional' on page 5 undefined on input
 line 1124.


LaTeX Warning: Citation `li2019massive' on page 5 undefined on input line 1124.


[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>]
(./draft.bbl)

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux)

LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `draft.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 768815 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 97).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 143). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;

Overfull \hbox (65.78949pt too wide) detected at line 963
[]
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] [5 <./figs/Fig.
rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>] (./draft.bbl)

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 769041 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 899
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;

Overfull \hbox (65.78949pt too wide) detected at line 965
[]

Underfull \vbox (badness 2990) has occurred while \output is active [4 <./figs/
Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] [5 <./figs/Fig.rmse_vs_anc
hors.pdf> <./figs/Fig.rmse_vs_noise.pdf>] (./draft.bbl)

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 768906 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 899
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;

Overfull \hbox (65.78949pt too wide) detected at line 965
[]

Underfull \vbox (badness 2990) has occurred while \output is active [4 <./figs/
Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] [5 <./figs/Fig.rmse_vs_anc
hors.pdf> <./figs/Fig.rmse_vs_noise.pdf>] (./draft.bbl)

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux)

LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 768811 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 899
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;

Overfull \hbox (65.78949pt too wide) detected at line 965
[]

Underfull \vbox (badness 2990) has occurred while \output is active [4 <./figs/
Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] [5 <./figs/Fig.rmse_vs_anc
hors.pdf> <./figs/Fig.rmse_vs_noise.pdf>] (./draft.bbl)

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 768747 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 899
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;

Overfull \hbox (65.78949pt too wide) detected at line 965
[]

Underfull \vbox (badness 2990) has occurred while \output is active [4 <./figs/
Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] [5 <./figs/Fig.rmse_vs_anc
hors.pdf> <./figs/Fig.rmse_vs_noise.pdf>] (./draft.bbl)

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 768519 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] (./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (1.73193pt too high) has occurred while \output is active
[6] (./draft.aux)

LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `draft.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.

 )
(see the transcript file for additional information)pdfTeX warning (dest): name
{equation.3.2} has been referenced but does not exist, replaced by a fixed one

{/usr/local/texlive/2021/texmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/tex
live/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texl
ive/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmex10.pfb></usr/local/texli
ve/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi10.pfb></usr/local/texliv
e/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/
2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/20
21/texmf-dist/fonts/type1/public/amsfonts/cm/cmmib10.pfb></usr/local/texlive/20
21/texmf-dist/fonts/type1/public/amsfonts/cmextra/cmmib7.pfb></usr/local/texliv
e/2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/
2021/texmf-dist/fonts/type1/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/202
1/texmf-dist/fonts/type1/public/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/t
exmf-dist/fonts/type1/public/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/te
xmf-dist/fonts/type1/public/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texm
f-dist/fonts/type1/public/amsfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-
dist/fonts/type1/public/amsfonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-di
st/fonts/type1/public/amsfonts/symbols/msbm10.pfb></usr/local/texlive/2021/texm
f-dist/fonts/type1/urw/times/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fon
ts/type1/urw/times/utmbi8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/
urw/times/utmr8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/
utmri8a.pfb>
Output written on draft.pdf (6 pages, 763984 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] (./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (1.73193pt too high) has occurred while \output is active
[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 763975 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] (./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (1.73193pt too high) has occurred while \output is active
[6] (./draft.aux)

LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 763778 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] (./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (1.73193pt too high) has occurred while \output is active
[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 763388 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 897
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] (./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (1.73193pt too high) has occurred while \output is active
[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 763388 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 898
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] (./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (1.73193pt too high) has occurred while \output is active
[6] (./draft.aux)

LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 763413 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Overfull \hbox (16.0748pt too wide) in paragraph at lines 595--597
 [][] 
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 898
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf> <./figs/Fig.detailed_level.pdf>] (./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.


Overfull \vbox (1.73193pt too high) has occurred while \output is active
[6] (./draft.aux) )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 763443 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Overfull \hbox (16.0748pt too wide) in paragraph at lines 595--597
 [][] 
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]
Overfull \hbox (16.22815pt too wide) detected at line 898
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf>]
Underfull \vbox (badness 6110) has occurred while \output is active
(./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux)

LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 725201 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Overfull \hbox (16.0748pt too wide) in paragraph at lines 595--597
 [][] 
[2 <./figs/Fig.ecc_icc.pdf>] [3 <./figs/Fig.city_map.pdf>]

LaTeX Warning: Reference `fig:low_level' on page 4 undefined on input line 865.



Overfull \hbox (16.22815pt too wide) detected at line 898
[][]\OML/cmm/m/it/10 C [] \OT1/cmr/m/n/10 = [] [] [] [][] \OML/cmm/m/it/10 ;
[4 <./figs/Fig.high_level.pdf>]
Underfull \vbox (badness 6110) has occurred while \output is active
(./draft.bbl

Package balance Warning: You have called \balance in second column
(balance)                Columns might not be balanced.

[5 <./figs/Fig.rmse_vs_anchors.pdf> <./figs/Fig.rmse_vs_noise.pdf>])

** Conference Paper **
Before submitting the final camera ready copy, remember to:

 1. Manually equalize the lengths of two columns on the last page
 of your paper;

 2. Ensure that any PostScript and/or PDF output post-processing
 uses only Type 1 fonts and that every step in the generation
 process uses the appropriate paper size.

[6] (./draft.aux)

LaTeX Warning: There were undefined references.

 )
(see the transcript file for additional information){/usr/local/texlive/2021/te
xmf-dist/fonts/enc/dvips/base/8r.enc}</usr/local/texlive/2021/texmf-dist/fonts/
type1/public/amsfonts/cm/cmbx10.pfb></usr/local/texlive/2021/texmf-dist/fonts/t
ype1/public/amsfonts/cm/cmex10.pfb></usr/local/texlive/2021/texmf-dist/fonts/ty
pe1/public/amsfonts/cm/cmmi10.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmmi5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmmi7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cm/cmmib10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/p
ublic/amsfonts/cmextra/cmmib7.pfb></usr/local/texlive/2021/texmf-dist/fonts/typ
e1/public/amsfonts/cm/cmr10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1
/public/amsfonts/cm/cmr5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/pu
blic/amsfonts/cm/cmr7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/publi
c/amsfonts/cm/cmsy10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public
/amsfonts/cm/cmsy5.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/a
msfonts/cm/cmsy7.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/ams
fonts/cm/cmsy8.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/public/amsfo
nts/symbols/msbm10.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/time
s/utmb8a.pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmbi8a.
pfb></usr/local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmr8a.pfb></usr/
local/texlive/2021/texmf-dist/fonts/type1/urw/times/utmri8a.pfb>
Output written on draft.pdf (6 pages, 725545 bytes).
Transcript written on draft.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.22 (TeX Live 2021) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./draft.tex
LaTeX2e <2020-10-01> patch level 4
L3 programming layer <2021-02-18> (./IEEEtran.cls
Document Class: IEEEtran 2007/03/05 V1.7a by Michael Shell
-- See the "IEEEtran_HOWTO" manual for usage information.
-- http://www.michaelshell.org/tex/ieeetran/
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/ot1ptm.fd)
-- Using 8.5in x 11in (letter) paper.
-- Using PDF output.
-- This is a 10 point document.
) (./include_v5.tex
(/usr/local/texlive/2021/texmf-dist/tex/latex/savesym/savesym.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/fixltx2e.sty

Package fixltx2e Warning: fixltx2e is not required with releases after 2015
(fixltx2e)                All fixes are now in the LaTeX kernel.
(fixltx2e)                See the latexrelease package for details.

) (/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/keyval.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/subcaption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/caption/caption3.sty)

Package caption Warning: Unknown document class (or package),
(caption)                standard defaults will be used.
See the caption package documentation for explanation.

)) (/usr/local/texlive/2021/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/calc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/amssymb.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/bm.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics/color.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/accents/accents.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/theoremref/theoremref.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/url/url.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hyperref-langpatches.def
) (/usr/local/texlive/2021/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2021/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2021/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2021/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2021/texmf-dist/tex/latex/algorithm2e/algorithm2e.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2021/texmf-dist/tex/latex/relsize/relsize.sty))
(/usr/local/texlive/2021/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
(./draft.aux)
(/usr/local/texlive/2021/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2021/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2021/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2021/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2021/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./draft.out) (./draft.out)
** WARNING: \thanks is locked out when in conference mode (line 100).
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2021/texmf-dist/tex/latex/psnfss/omsptm.fd)
** ATTENTION: \keywords is deprecated (line 146). Use \IEEEkeywords instead.
[1{/usr/local/texlive/2021/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Overfull \hbox (16.0748pt too wide) in paragraph at lines 595--597
 [][] 
[2 <./figs/Fig.ecc_icc.pdf>]
! Missing number, treated as zero.
<to be read again> 
                   }
l.833 \begin{figure}[b]{\linewidth}
                                   
? 
! Emergency stop.
<to be read again> 
                   }
l.833 \begin{figure}[b]{\linewidth}
                                   
!  ==> Fatal error occurred, no output PDF file produced!
Transcript written on draft.log.

